Metric Based Few-Shot Graph Classification

Many modern deep-learning techniques do not work without enormous datasets. At the same time, several fields demand methods working in scarcity of data. This problem is even more complex when the samples have varying structures, as in the case of graphs. Graph representation learning techniques have recently proven successful in a variety of domains. Nevertheless, the employed architectures perform miserably when faced with data scarcity. On the other hand, few-shot learning allows employing modern deep learning models in scarce data regimes without waiving their effectiveness. In this work, we tackle the problem of few-shot graph classification, showing that equipping a simple distance metric learning baseline with a state-of-the-art graph embedder allows to obtain competitive results on the task. While the simplicity of the architecture is enough to outperform more complex ones, it also allows straightforward additions. To this end, we show that additional improvements may be obtained by encouraging a task-conditioned embedding space. Finally, we propose a MixUp-based online data augmentation technique acting in the latent space and show its effectiveness on the task.

==> 1_Introduction/root_old.tex <==
% Intro to GRL
In the past few years, Graph Representation Learning techniques (cite main works) have resulted in significant improvements in many fields where network-structured data is abundant. Moreover, their flexibility has allowed these models to be effectively employed in different domains such as Computer Vision (CV) (cite..) and Natural Language Processing (NLP) (cite..). 
% Scarce data problem
Nevertheless, as most deep learning models, their expressivity comes at a cost: the complex hypothesis spaces they define result in a large number of parameters, which in turn require vast amounts of data to be tuned. When data is instead scarce, these models end up capturing noise in the training data, hindering their performance on unseen samples.
Supervised samples for graph-structured data are particularly hard to obtain, as the annotation process is often expensive in time and resources \cite{adv-graph-augm, pretraining-gnns, infograph}.
This is particularly true when the samples come from specialized domains such as biology, chemistry and medicine (CITE crossdomain FS-GC), where graph-structured data are very common. Drug testing, for instance, requires expensive in-vivo experiments for a drug to be labelled. Analogously, laborious wet experiments are required to label protein graphs (CITE AS-MAML).

% FSL
In general, the field of Few-Shot Learning (FSL) (cite ...) aims at designing models which can effectively operate in scarce data scenarios.
% Task
While there has been some interest in Few-Shot Node Classification and Link Prediction, Graph-level classification has mostly been overlooked in the Few-Shot setting.
% Proposal
Fortunately, leveraging recent highly-expressive graph embedding techniques, several of the FSL techniques employed in Computer Vision can be adapted to the graph setting with minor modifications.
To this end, we propose adapting Prototypical Networks \cite{PrototypicalNets} to graph-structured data, a simple-yet-effective Distance Metric Learning approach that has been obtained remarkable results in CV. 
We then show that it is enough to obtain competitive results in the task when equipped with a state-of-the-art graph embedder.

% Episode-conditioned embedding space
As it is often the case in DML architectures for FSL, the architecture is not optimized over the novel samples, but is only able to discriminate them thanks to the generality of its learned embedding space. 
Nevertheless, the same embedding space may not be fit for discriminating all pairs of classes, as certain features may be pivotal in a case and less important in another.
Believing the considerations made in \cite{TADAM} to be modality-agnostic, we also follow their suggestion to equip ProtoNet with an episode-conditioning module. The latter modulates the intermediate representations in function of the particular episode.

% Regularizer
A major difficulty of FSL stems from the fact that supervised data is insufficient to allow learning meaningful features for the task from scratch. A learning model must therefore learn general features from some other data distribution and adapt them to the data-scarce task.
This means that the representations for the novel classes will mostly be a rearrangement of those from the data-abundant base classes.
To this end, we propose employing a novel online data augmentation technique that creates novel samples from two support samples as a mixup of their latent representations, this way training the model to expect combinations of the base samples already at training time, encouraging more general features that are useful to overcome the limited data availability.

% Contributions
Our contribution is three-fold:
\begin{enumerate}
    \item Show that a simple DML baseline works better than more complex meta-learning approaches for the task of Few-Shot Graph Classification;
    \item Equip the architecture with an episode-adaptive module and show that it is beneficial for the task;
    \item We suggest a novel online data augmentation technique that creates new artificial samples in the latent space, and show that it provides a significant gain in performance.
\end{enumerate}
%
\begin{figure}
    \centering
    \includegraphics{figures/episode.png}
    \caption{An $N$-way $K$-shot episode. (...) (TO BE ADAPTED TO THE PAPER AND RECOLOURED)}
    \label{fig:episode}
\end{figure}
